On closed P-sets with ccc in the space omega^*

It is proved that -- consistently -- there can be no ccc closed P-sets in the remainder space omega^* .

==> mssymb.tex <==

\message{Not using the real mssymb file}
\message{Inputting amssym.def and amssym.tex instead}
 {\catcode`\@11 \global\def\setboxz@h{\setbox0\hbox}
	\global\def\wdz@{\wd0 }
 }

\input amssym.def
\input amssym.tex
\def\napprox{\not\approx}

